NetRep: Automatic Repair for Network Programs

Debugging imperative network programs is a challenging task for developers because understanding various network modules and complicated data structures is typically time-consuming. To address the challenge, this paper presents an automated technique for repairing network programs from unit tests. Specifically, given as input a faulty network program and a set of unit tests, our approach localizes the fault through symbolic reasoning, and synthesizes a patch such that the repaired program can pass all unit tests. It applies domain-specific abstraction to simplify network data structures and utilizes modular analysis to facilitate function summary reuse for symbolic analysis. We implement the proposed techniques in a tool called NetRep and evaluate it on 10 benchmarks adapted from real-world software-defined networking controllers. The evaluation results demonstrate the effectiveness and efficiency of NetRep for repairing network programs.

==> algo-select.tex <==
\begin{figure}[!t]
\begin{algorithm}[H]
\caption{Function Selection}
\label{algo:select}
\begin{algorithmic}[1]
\Procedure{\textsc{SelectFunction}}{$\prog, \visited$}
\vspace{2pt}
\small
\Statex \textbf{Input:} Program $\prog$, visited map $\visited$
\Statex \textbf{Output:} Function $\func$ or $\bot$ to indicate failure

\State $\func' \gets \textsf{MainFunc}(\prog)$;
\While{$\func' \neq \bot$}
    \State $\func \gets \func'$;
    \State $\func' \gets \textsc{GetActiveCallee}(\prog, \visited, \func)$;
\EndWhile
\State \Return $\func$;
\EndProcedure

\Procedure{\textsc{GetActiveCallee}}{$\prog, \visited, \func$}
\vspace{2pt}
\small
\Statex \textbf{Input:} Program $\prog$, visited map $\visited$, function $\func$
\Statex \textbf{Output:} Active callee $\func'$ or $\bot$ to indicate failure

\State $\mathcal{F} \gets \textsf{GetCallees}(\prog, \func)$;
\For{\textbf{each} $\func' \in \mathcal{F}$}
    \State $\lineid \gets \textsf{GetCallSite}(\prog, \func, \func')$;
    \If{$\visited[\lineid] = \emph{true}$ \textbf{and} $\exists \lineid'.~ \textsf{TransInFunc}(\lineid', \prog, \func) \land \visited[\lineid'] = \emph{false}$}
        \State \Return $\func'$;
    \EndIf
\EndFor
\State \Return $\bot$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-10pt}
\end{figure}

